ACTI at EVALITA 2023: Overview of the Conspiracy Theory Identification Task

Conspiracy Theory Identication task is a new shared task proposed for the first time at the Evalita 2023. The ACTI challenge, based exclusively on comments published on conspiratorial channels of telegram, is divided into two subtasks: (i) Conspiratorial Content Classification: identifying conspiratorial content and (ii) Conspiratorial Category Classification about specific conspiracy theory classification. A total of fifteen teams participated in the task for a total of 81 submissions. We illustrate the best performing approaches were based on the utilization of large language models. We finally draw conclusions about the utilization of these models for counteracting the spreading of misinformation in online platforms.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> commenting.tex <==
\usepackage{bbm}
\usepackage{todonotes}
%\usepackage[disable]{todonotes}
\makeatletter
\newcommand*\iftodonotes{\if@todonotes@disabled\expandafter\@secondoftwo\else\expandafter\@firstoftwo\fi}  % defines \iftodonotes{<true>}{<false>}, thanks to https://tex.stackexchange.com/questions/126559/conditional-based-on-packageoption
\makeatother
\newcommand{\noindentaftertodo}{\iftodonotes{\noindent}{}}
% Note that these macros accept optional arguments such as size=\small, bordercolor=red, and so on.  Capitalized versions are inline paragraphs instead of margin notes.
\newcommand{\fixme}[2][]{\todo[color=yellow,size=\scriptsize,fancyline,caption={},#1]{#2}} % to mark stuff that you know is missing or wrong when you write the text
\newcommand{\note}[4][]{\todo[author=#2,color=#3,size=\scriptsize,fancyline,caption={},#1]{#4}} % default note settings, used by macros below.

\newcommand{\notewho}[3][]{\note[#1]{#2}{blue!40}{#3}}     % for other commenters: specify author name in first required arg
\newcommand{\Fixme}[2][]{\fixme[inline,#1]{#2}\noindentaftertodo}
\newcommand{\Notewho}[3][]{\notewho[inline,#1]{#2}{#3}\noindentaftertodo}
\newcommand{\rajarshi}[2][]{\note[#1]{rajarshi}{purple!60}{#2}}
\newcommand{\Rajarshi}[2][]{\rajarshi[inline,#1]{#2}\noindentaftertodo}
\newcommand{\pengxiang}[2][]{\note[#1]{pengxiang}{red!60}{#2}}
\newcommand{\Pengxiang}[2][]{\pengxiang[inline,#1]{#2}\noindentaftertodo}

\newcommand{\nik}[2][]{\note[#1]{nik}{orange!60}{#2}}
\newcommand{\Nik}[2][]{\nik[inline,#1]{#2}\noindentaftertodo}
\newcommand{\response}[1]{\vspace{3pt}\hrule\vspace{3pt}\textbf{#1:} }
\newcommand{\NikEdit}[1]{{\color{red} #1}}


%%%%%%%%%%%% TEXT
\newcommand{\needref}{({\color{orange} ref})}
\newcommand{\needcite}{({\color{red} cite})}
\newcommand{\needcitefor}[1]{({\color{red} #1})}
\newcommand{\fillin}{({\color{blue} fill-in})}
\newcommand{\fillinwith}[1]{({\color{blue} #1})}


\usepackage{tipa}
\newcommand{\ucambridge}{\normalfont \text{\textipa{D}}}
\newcommand{\ethz}{\text{\normalfont \textipa{Q}}}
\newcommand{\mitinst}{\normalfont \text{\textipa{@}}}
\newcommand{\epfl}{\normalfont \text{\textipa{N}}}
\newcommand{\bloomberg}{\normalfont \text{\textipa{R}}}
